Thought experiments in a quantum computer

We introduce a software package that allows users to design and run simulations of thought experiments in quantum theory. In particular, it covers cases where several reasoning agents are modelled as quantum systems, such as Wigner's friend experiment. Users can customize the protocol of the experiment, the inner workings of agents (including a quantum circuit that models their reasoning process), the abstract logical system used (which may or not allow agents to combine premises and make inferences about each other's reasoning), and the interpretation of quantum theory used by different agents. Our open-source software is written in a quantum programming language, ProjectQ, and runs on classical or quantum hardware. As an example, we model the Frauchiger-Renner extended Wigner's friend thought experiment, where agents are allowed to measure each other's physical memories, and make inferences about each other's reasoning.

==> pictures/thoughtexperiment.tex <==
The aim of this section is to give the reader the idea and intuition behind the Frauchiger-Renner thought experiment \cite{Frauchiger2018}; we will focus on the exact way we model it later in the paper. The setting of the experiment consists of four agents: Alice, Bob, Ursula and Wigner. Each experimenter is equipped with a memory qubit ($A, B, U$ and $W$, respectively). Additionally, there are two other systems - qubits $R$ and $S$.

The initial state of the $R$ is $\sqrt{\frac{1}{3}}\ket{0}_R+\sqrt{\frac{2}{3}}\ket{1}_R$. The initial state of $S$ is $\ket{0}_S$. The initial state of the relevant subsystems of the agents' memories is $\ket0_A, \ket0_B, \ket0_U $ and $\ket0_W$. 
The experiment proceeds as follows: 
\begin{enumerate}[{$t= $} 1.]
    \item Alice measures system $R$ in basis $\{\ket0_R, \ket1_R\}$. She records the result in her memory $A$, and prepares $S$ accordingly: if she obtains outcome $a=0$ she keeps her memory in state $\ket0_A$ and $S$ in state $\ket0_S$; if she obtains outcome $a=1$ she changes her memory to  $\ket1_A$ and $S$ to $\frac1{\sqrt2}(\ket0_S+\ket1_S)$. Thus, first the joint state of $R$ and her memory $A$ becomes entangled,
    \begin{gather*}
    \left(\sqrt{\frac{1}{3}}\ket{0}_R+\sqrt{\frac{2}{3}}\ket{1}_R\right)\ket{0}_A 
    \quad \longrightarrow \quad
    \sqrt{\frac{1}{3}}\ket{0}_R\ket{0}_A+\sqrt{\frac{2}{3}}\ket{1}_R\ket{1}_A.
    \end{gather*}
    When Alice prepares $S$, it too becomes entangled with $R$ and $A$,
     \begin{gather*}
    \sqrt{\frac{1}{3}}\ket{0}_R\ket{0}_A \ket0_S+\sqrt{\frac{2}{3}}\ket{1}_R\ket{1}_A \  \frac1{\sqrt2}(\ket0_S +\ket1_S).
    \end{gather*}
    Alice sends $S$ to Bob.
    
    \item Bob measures system $S$ in basis $\{\ket0_S, \ket1_S\}$ and records the outcome $b$ in his memory $B$, similarly to Alice. The global state of $R$, $A$, $S$ and $B$ becomes
    \begin{gather*}
    \ket{\psi}_{RASB} = \frac{1}{\sqrt{3}}\left(\ket{0}_R\ket{0}_A \ket0_S\ket0_B+ \ket{1}_R\ket{1}_A\ket0_S\ket0_B +\ket{1}_R\ket{1}_A\ket1_S\ket1_B \right).
    \end{gather*}
    
    \item Ursula measures Alice's lab (consisting of $R$ and the memory $A$) in basis $\{\ket{ok}_{RA}, \ket{fail}_{RA}\}$, where
    \begin{gather*}
    \ket{ok}_{RA}=\sqrt{\frac{1}{2}}(\ket{0}_R\ket{0}_A-\ket{1}_R\ket{1}_A)\\
    \ket{fail}_{RA}=\sqrt{\frac{1}{2}}(\ket{0}_R\ket{0}_A+\ket{1}_R\ket{1}_A).
    \end{gather*}

    \item Wigner measures Bob's lab (consisting of $S$ and the memory $B$) in basis $\{\ket{ok}_{SB}, \ket{fail}_{SB}\}$, where
    \begin{gather*}
    \ket{ok}_{SB}=\sqrt{\frac{1}{2}}(\ket{0}_S\ket{0}_B-\ket{1}_S\ket{1}_B)\\
    \ket{fail}_{SB}=\sqrt{\frac{1}{2}}(\ket{0}_S\ket{0}_B+\ket{1}_S\ket{1}_B).
    \end{gather*}

    \item Ursula and Wigner compare the outcomes of their measurements. If they were both ``ok'', they halt the experiment. Otherwise, they reset the timer and all systems to the initial conditions, and repeat the experiment. If we follow the Born rule, this experiment will at some point halt, as the overlap of the global state at time $t=2.5$ with $\ket{ok}_{RA}\ket{ok}_{SB}$ gives us a probability of $1/12$.
\end{enumerate}

It can be shown that since the global state $\ket{\psi}_{RASB}$ can be rewritten as $$\frac{1}{\sqrt{3}}\ket{0}_R\ket{0}_A \ket0_S\ket0_B + \sqrt{\frac{2}{3}} \ket1_R\ket1_A \ket{fail}_{SB},$$ Alice can reason that whenever she finds $R$ in state $\ket1_R$, Wigner will obtain outcome ``fail'' when he measures Bob's lab. In other words, the inference ``$a=1 \implies w=fail$'' can be made. Analogously, one can derive inferences ``$b=1 \implies a=1$'' and ``$u=ok \implies b=1$'' made by Bob and Ursula respectively.
Together with both Ursula and Wigner eventually obtaining ``ok'', chaining these statements leads to a contradiction: given that Wigner got an outcome ``ok'', he with certainty predicts that he got outcome ``fail''.

This result is derived under following assumptions: 
\begin{enumerate}
    \item (Q) Agents use a weaker version of Born rule, applicable only to deterministic outcomes, to formulate their predictions;
    \item (S) Agents experience only one outcome;
    \item (C) Agents reason from viewpoints of each other;
    \item (U) Agents assume unitary evolution in each others labs.
\end{enumerate}

Further discussion on the assumptions can be found in \cite{Frauchiger2018, NL2018}.



